The strong coupling constant: State of the art and the decade ahead

Theoretical predictions for particle production cross sections and decays at colliders rely heavily on perturbative Quantum Chromodynamics (QCD) calculations, expressed as an expansion in powers of the strong coupling constant $\alpha_s$. The current $\mathcal{O}(1\%)$ uncertainty of the QCD coupling evaluated at the reference Z boson mass, $\alpha_s(m_Z) = 0.1179 \pm 0.0009$, is one of the limiting factors to more precisely describe multiple processes at current and future colliders. A reduction of this uncertainty is thus a prerequisite to perform precision tests of the Standard Model as well as searches for new physics. This report provides a comprehensive summary of the state-of-the-art, challenges, and prospects in the experimental and theoretical study of the strong coupling. The current $\alpha_s(m_Z)$ world average is derived from a combination of seven categories of observables: (i) lattice QCD, (ii) hadronic $\tau$ decays, (iii) deep-inelastic scattering and parton distribution functions fits, (iv) electroweak boson decays, hadronic final-states in (v) $e^+e^-$, (vi) e-p, and (vii) p-p collisions, and (viii) quarkonia decays and masses. We review the current status of each of these seven $\alpha_s(m_Z)$ extraction methods, discuss novel $\alpha_s$ determinations, and examine the averaging method used to obtain the world-average value. Each of the methods discussed provides a ``wish list'' of experimental and theoretical developments required in order to achieve the goal of a per-mille precision on $\alpha_s(m_Z)$ within the next decade.

==> alphaS_intro.tex <==
\section{Introduction}
\label{sec:intro}
%\textcolor{red}{main editors: }


The strong coupling $\alphas$ is one of the fundamental parameters of the Standard Model (SM), setting the scale of the strength of the strong interaction theoretically described by Quantum Chromodynamics (QCD). Its value at the reference Z pole mass scale amounts to
$\alphasmZ$~=~0.1179~$\pm$~0.0009~\cite{ParticleDataGroup:2020ssz}, with a $\delta\alphas/\alphas \approx 0.85\%$ uncertainty that is orders of magnitude larger than that of any other fundamental coupling in nature. Improving our knowledge of $\alphas$ is crucial, among other things, to reduce the theoretical uncertainties in the  high-precision calculations of all perturbative QCD (pQCD) processes whose cross sections or decay rates depend on higher-order powers of $\alphas$, as is the case for virtually all those measured at the LHC. In the Higgs sector, our imperfect knowledge of $\alphas$ (combined with that of the charm mass) propagates today into total final uncertainties of $\sim$4\%??? for the H\,$\to gg\,(\ccbar)$ partial width(s). In the electroweak sector, the input $\alphasmZ$ value is the leading source of uncertainty in the calculation of crucial precision pseudoobservables such as the Z boson width and its Z\,$\to \bbbar$ (and other hadronic) decays. The QCD coupling plays also a fundamental role in the calculation of key quantities in top-quark physics, such as the top mass, width, and Yukawa coupling.\\

The workshop {\it ``\,$\alphas$(2022) -- Precision measurements of the QCD coupling''} was held at ECT*-Trento in Jan. 31st to Feb. 4th, 2022 (\ttt{http://indico.cern.ch/e/alphas2022}) with the aim of bringing together experts from various fields to explore in depth the latest developments on the determination of $\alphas$ from the key categories where high precision measurements and theoretical calculations are currently available. The meeting is the fourth of a ``series'' that started in Munich (Feb.~2011)~\cite{Proceedings:2011zvx},
%\href{https://arxiv.org/abs/1110.0016}{{\tt https://arxiv.org/abs/1110.0016}}), 
followed by
%{\it ``High-Precision $\alphas$ Measurements from LHC to FCC-ee''} (
CERN (Oct. 2015)~\cite{Proceedings:2015eho}, %\href{https://arxiv.org/abs/1512.05194}{{\tt https://arxiv.org/abs/1512.05194}}), 
and %{\it ``\,$\alphas$(2019) -- Precision measurements of the QCD coupling''}
ECT*-Trento (Feb.~2019)~\cite{Proceedings:2019pra}. %(\ttt{http://indico.cern.ch/e/alphas2019})


\clearpage

Each contributor is requested to provide 1--3 pages of text/tables/figures summarizing their workshop presentation with relevant bibliography and, in particular, addressing the following questions :
\begin{enumerate}
\item 1) Overarching questions: What is the current state-of-the-art and the ultimate theoretical \& experimental precision for your favourite $\alphas$ extraction method? What do we need to achieve such ultimate precision?
\item 2) Theory: What is the situation with the higher-order corrections (pQCD, mixed QCD-EW) for your $\alphas$ favourite observable? What is the impact of non-pQCD corrections/uncertainties? (Are there new techniques to reduce them?) Provide your personal wish-list in data/theory developments needed to reach your ultimate $\alphas$ precision.
\item 3) Experiment: What are the current leading syst./stat. uncertainties for your favourite observable? What are the expected future syst./stat. reductions with current \& future (e+e-, e-p, p-p) machines? (Are there new observables being considered?) Provide your personal wish-list in data/theory developments needed to reach your ultimate $\alphas$ precision.
\end{enumerate}


